Faster Convergence in Multi-Objective Optimization Algorithms Based on Decomposition

The Resource Allocation approach (RA) improves the performance of MOEA/D by maintaining a big population and updating few solutions each generation. However, most of the studies on RA generally focused on the properties of different Resource Allocation metrics. Thus, it is still uncertain what the main factors are that lead to increments in performance of MOEA/D with RA. This study investigates the effects of MOEA/D with the Partial Update Strategy in an extensive set of MOPs to generate insights into correspondences of MOEA/D with the Partial Update and MOEA/D with small population size and big population size. Our work undertakes an in-depth analysis of the populational dynamics behaviour considering their final approximation Pareto sets, anytime hypervolume performance, attained regions and number of unique non-dominated solutions. Our results indicate that MOEA/D with Partial Update progresses with the search as fast as MOEA/D with small population size and explores the search space as MOEA/D with big population size. MOEA/D with Partial Update can mitigate common problems related to population size choice with better convergence speed in most MOPs, as shown by the results of hypervolume and number of unique non-dominated solutions, the anytime performance and Empirical Attainment Function indicates.

==> files/bios.tex <==

% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Yuri Lavinas}}]{Yuri Lavinas}
% is a PhD student at the University of Tsukuba. He graduated in Computer Science (2016) in the University of Brasilia, Brazil, and got his Master Degree at the University of Tsukuba (2020). His research focus on Multi Objective Evolutionary Computation, neuro-evolution and Artificial Life. 
% \end{IEEEbiography}

% if you will not have a photo at all:
% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Claus Aranha}}]{Claus Aranha}
% obtained his PhD from the University of Tokyo in 2010, and is currently 
% an assistant professor at the University of Tsukuba, and a member of the
% Center for Artificial Intelligence (C-AIR). His research focus on the study 
% and application of Evolutionary Computation, including optimization, 
% procedural generation, and artificial life simulations.
% \end{IEEEbiography}

% insert where needed to balance the two columns on the last page with
% biographies

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Marcelo Ladeira }}]{Marcelo Ladeira} has a DSc degreee in Computer Science 
% from the Federal University of Rio Grande do Sul (1999), a 
% Post-doctorate at the University of Lisbon (2004), and 
% currently is a associate professor at the University of Brasilia. 
% He has experience on the study and development of application 
% in the area of Computer Science, with emphasis 
% in the subjects: Probabilistic Network Models, Data Science and Evolutionary Computation.
% \end{IEEEbiography}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}


==> files/hv_means.tex <==
\begin{table}[tbp]
\vspace{-2.85em}
\centering
\scriptsize
\caption[Means and standard errors for HV.]{Means (standard errors) for HV and proportion of nondominated solutions, for each problem. Best results are highlighted in bold.}
\vspace{-1.55em}
\label{chap5:stats_bibbob_hv}
\begin{tabular}[t]{c||c|c|c||c|c|c}
    
    \rowcolor[gray]{.8} \multicolumn{4}{c||}{\textbf{HV}} &\multicolumn{3}{c}{\textbf{NNDOM}}\\ \hline 
    \rowcolor[gray]{.9} MOP & MOEA/D-PS & Big population & Small population & MOEA/D-PS & Big population & Small population \\ \hline 
% \rowcolor[gray]{.95} DTLZ problems & MOEA/D-PS = 50 & Big pop. & Small pop. \\ \hline 
DTLZ1              & \textbf{1.00 (0.01)} &\textbf{1.00 (0.00)} & \textbf{1.00 (0.00)} & \textbf{1.00 (0.00) }&0.13 (0.08) &0.66 (0.25)\\
DTLZ2              & \textbf{0.99 (0.00)} &\textbf{0.99 (0.00)} &\textbf{0.99 (0.00)} &\textbf{0.99 (0.02)} &0.95 (0.02) &0.92 (0.05)\\
DTLZ3              & \textbf{1.00 (0.01)} &\textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} &\textbf{0.99 (0.01)} &0.11 (0.13) &0.80 (0.20)\\
DTLZ4              & \textbf{0.99 (0.00)} &\textbf{0.99 (0.00)} &\textbf{0.99 (0.00)} &\textbf{0.99 (0.02)} &0.88 (0.05) &0.91 (0.05)\\

\rowcolor[gray]{.95}DTLZ1$^{-1}$ & 0.44 (0.02) &0.35 (0.01) &\textbf{0.46 (0.01)}& \textbf{1.00 (0.00)} &0.29 (0.04) &0.98 (0.02)\\
\rowcolor[gray]{.95}DTLZ2$^{-1}$          & \textbf{0.78 (0.00)} &\textbf{0.78 (0.00)} &0.77 (0.00)& \textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} &\textbf{1.00 (0.01)}\\
\rowcolor[gray]{.95}DTLZ3$^{-1}$ & \textbf{0.75 (0.01)} &0.60 (0.03) & \textbf{0.75 (0.01)}& \textbf{1.00 (0.00)} &0.17 (0.03) &0.96 (0.03)\\
\rowcolor[gray]{.95}DTLZ4$^{-1}$          & \textbf{0.78 (0.00)} &\textbf{0.78 (0.00)} &0.77 (0.00)& \textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} &0.99 (0.01)\\

UF1       & 0.94 (0.02) &\textbf{0.98 (0.00)} &0.95 (0.02) & \textbf{0.96 (0.04)} &0.37 (0.06) &0.54 (0.07)\\
UF2       & 0.92 (0.01) &\textbf{0.94 (0.01)} &\textbf{0.94 (0.01)} & \textbf{0.98 (0.03)} & 0.38 (0.05) &0.54 (0.04)\\
UF3       & 0.91 (0.03) &\textbf{0.98 (0.00)} &0.96 (0.03) & \textbf{0.97 (0.04)} &0.24 (0.03) &0.53 (0.09)\\
UF4       & 0.48 (0.00) &\textbf{0.50 (0.00)} &0.47 (0.01) & \textbf{0.96 (0.04)} &0.56 (0.05) &0.73 (0.07)\\
UF5       & 0.90 (0.04) &\textbf{0.96 (0.01)} &0.90 (0.03) & \textbf{0.78 (0.20)} &0.20 (0.03) &0.44 (0.10)\\
UF6       & 0.92 (0.04) &\textbf{0.97 (0.00)} &0.93 (0.05) & \textbf{0.96 (0.04)} &0.31 (0.05) &0.50 (0.06)\\
UF7       & 0.92 (0.08) &\textbf{0.97 (0.00)} &0.94 (0.06) & \textbf{0.93 (0.21)} &0.48 (0.08) &0.61 (0.11)\\
UF8                & 0.99 (0.00) &\textbf{1.00 (0.00)} &0.99 (0.00) & \textbf{0.99 (0.01)} &0.64 (0.09) &0.79 (0.05)\\
UF9                & \textbf{0.99 (0.00)} &\textbf{0.99 (0.00)} &\textbf{0.99 (0.00)} & \textbf{0.99 (0.01)} &0.60 (0.12) &0.70 (0.10)\\
UF10      & \textbf{0.98 (0.01)} &\textbf{0.98 (0.00)} &0.97 (0.01) & \textbf{0.93 (0.08)} &0.46 (0.04) &0.73 (0.08)\\

\rowcolor[gray]{.95}F1         & \textbf{0.96 (0.00)} &\textbf{0.96 (0.01)} &\textbf{0.96 (0.00)} & \textbf{0.99 (0.01)} &0.32 (0.06) &0.50 (0.04)\\
\rowcolor[gray]{.95}F2         & \textbf{1.00 (0.01)} &0.99 (0.00) &\textbf{1.00 (0.00)} & \textbf{0.99 (0.01)} &0.29 (0.06) &0.54 (0.08)\\
\rowcolor[gray]{.95}F3                  & \textbf{0.98 (0.00)} &\textbf{0.98 (0.00)} &\textbf{0.98 (0.00)} & \textbf{1.00 (0.01)} &0.36 (0.05) &0.58 (0.04)\\
\rowcolor[gray]{.95}F4                  & \textbf{1.00 (0.00)} &0.99 (0.00) &\textbf{1.00 (0.00)} & \textbf{0.99 (0.01)} &0.25 (0.05) &0.47 (0.07)\\
\rowcolor[gray]{.95}F5         & 0.91 (0.01) &0.90 (0.01) &\textbf{0.93 (0.00)} & \textbf{0.99 (0.01)} &0.33 (0.03) &0.49 (0.06)\\
\rowcolor[gray]{.95}F6                  & 0.99 (0.00) &0.99 (0.00) &\textbf{1.00 (0.00)} & \textbf{0.99 (0.01)} &0.25 (0.05) &0.51 (0.06)\\
\rowcolor[gray]{.95}F7                  & 0.99 (0.00) &0.99 (0.00) &\textbf{1.00 (0.00)} & \textbf{0.99 (0.01)} &0.18 (0.02) &0.37 (0.07)\\
\rowcolor[gray]{.95}F8                  & \textbf{0.99 (0.00)} &\textbf{0.99 (0.00)} &\textbf{0.99 (0.00)} & \textbf{0.89 (0.11)} &0.16 (0.01) &0.42 (0.11)\\
\rowcolor[gray]{.95}F9                  & \textbf{1.00 (0.00)} &0.99 (0.00) &\textbf{1.00 (0.00)} & \textbf{0.99 (0.01)} &0.31 (0.06) &0.54 (0.09)\\
\rowcolor[gray]{.95}F10        & 0.79 (0.03) &\textbf{0.80 (0.00)} &0.77 (0.05) & \textbf{0.99 (0.01)} &0.45 (0.07) &0.55 (0.05)\\
\rowcolor[gray]{.95}F11                 & \textbf{0.98 (0.00)} &\textbf{0.98 (0.00)} &\textbf{0.98 (0.00)} & \textbf{0.99 (0.01)} &0.31 (0.06) &0.55 (0.06)\\
\rowcolor[gray]{.95}F12                          & \textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} & \textbf{0.96 (0.04)} &0.29 (0.05) &0.62 (0.06)\\
\rowcolor[gray]{.95}F13                          & \textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} & \textbf{0.99 (0.01)} &0.27 (0.05) &0.53 (0.07)\\
\rowcolor[gray]{.95}F14        & 0.95 (0.01) &0.95 (0.01) &\textbf{0.98 (0.01)} & \textbf{0.99 (0.02)} &0.30 (0.05) &0.48 (0.05)\\
\rowcolor[gray]{.95}F15                          & \textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} & \textbf{0.99 (0.01)} &0.28 (0.04) &0.49 (0.05)\\
\rowcolor[gray]{.95}F16                 & 0.99 (0.00) &\textbf{1.00 (0.00)} &0.99 (0.00) & \textbf{0.99 (0.01)} &0.17 (0.01) &0.41 (0.14)\\
\rowcolor[gray]{.95}F17        & 0.99 (0.01) &\textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} & \textbf{0.94 (0.05)} &0.15 (0.02) &0.39 (0.10)\\
\rowcolor[gray]{.95}F18                          & \textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} & \textbf{0.99 (0.01)} &0.31 (0.04) &0.54 (0.09)\\
\rowcolor[gray]{.95}F19        & 0.93 (0.07) &\textbf{0.96 (0.02)} &0.93 (0.04) & \textbf{0.99 (0.02)} &0.40 (0.07) &0.62 (0.08)\\
\rowcolor[gray]{.95}F20                          & \textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} & \textbf{0.98 (0.02)} &0.43 (0.12) &0.66 (0.07)\\
\rowcolor[gray]{.95}F21                          & \textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} & \textbf{0.99 (0.02)} &0.28 (0.06) &0.56 (0.07)\\
\rowcolor[gray]{.95}F22        & 0.92 (0.03) &\textbf{0.96 (0.01)} &\textbf{0.96 (0.02)} & \textbf{0.99 (0.02)} &0.33 (0.06) &0.55 (0.06)\\
\rowcolor[gray]{.95}F23                          & \textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} & \textbf{0.99 (0.01)} &0.31 (0.04) &0.54 (0.04)\\
\rowcolor[gray]{.95}F24                 & 0.99 (0.00) &\textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} & \textbf{0.96 (0.04)} &0.16 (0.02) &0.39 (0.07)\\
\rowcolor[gray]{.95}F25                 & 0.99 (0.00) &\textbf{1.00 (0.00)} &0.99 (0.00) & \textbf{0.92 (0.10)} &0.14 (0.02) &0.32 (0.07)\\
\rowcolor[gray]{.95}F26                          & \textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} & \textbf{0.98 (0.02)} &0.37 (0.10) &0.70 (0.13)\\
\rowcolor[gray]{.95}F27        & 0.90 (0.07) &\textbf{0.94 (0.02)} &0.90 (0.06) & \textbf{0.99 (0.01)} &0.37 (0.05) &0.62 (0.06)\\
\rowcolor[gray]{.95}F28                          & \textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} & \textbf{0.99 (0.02)} &0.24 (0.06) &0.47 (0.08)\\
\rowcolor[gray]{.95}F29        & 0.96 (0.01) &0.96 (0.01) &\textbf{0.98 (0.00)} & \textbf{0.99 (0.02)} &0.24 (0.05) &0.44 (0.05)\\
\rowcolor[gray]{.95}F30                          & \textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} & \textbf{0.99 (0.02)} &0.27 (0.05) &0.45 (0.06)\\

\rowcolor[gray]{.95}F31        & 0.98 (0.01) &\textbf{1.00 (0.00) }&0.99 (0.00)  & \textbf{0.96 (0.07)} &0.16 (0.03) &0.42 (0.12)\\
\rowcolor[gray]{.95}F32                 & 0.99 (0.00) &\textbf{1.00 (0.00)} &0.99 (0.00)  & \textbf{0.95 (0.06)} &0.14 (0.02) &0.34 (0.06)\\
\rowcolor[gray]{.95}F33                          & \textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} & \textbf{0.99 (0.02)} &0.25 (0.03) &0.56 (0.12)\\
\rowcolor[gray]{.95}F34        & 0.94 (0.02) &0.94 (0.01) &\textbf{0.95 (0.02)} & \textbf{0.99 (0.02)} &0.35 (0.11) &0.50 (0.05)\\
\rowcolor[gray]{.95}F35        & 0.78 (0.02) &0.81 (0.01) &\textbf{0.82 (0.01)} & \textbf{0.99 (0.01)} &0.40 (0.06) &0.55 (0.04)\\
\rowcolor[gray]{.95}F36        & 0.91 (0.03) &\textbf{0.97 (0.01)} &0.98 (0.02) & \textbf{0.99 (0.01)} &0.30 (0.04) &0.52 (0.05)\\
\rowcolor[gray]{.95}F37        & 0.89 (0.02) &0.96 (0.01) &\textbf{0.97 (0.01)} & \textbf{0.98 (0.02)} &0.21 (0.03) &0.42 (0.03)\\
\rowcolor[gray]{.95}F38        & 0.91 (0.03) &0.96 (0.02) &\textbf{0.97 (0.02)} & \textbf{0.91 (0.12)} &0.18 (0.05) &0.39 (0.06)\\
\rowcolor[gray]{.95}F39        & 0.94 (0.01) &0.95 (0.01) &\textbf{0.97 (0.01)} & \textbf{0.99 (0.01)} &0.33 (0.05) &0.53 (0.07)\\
\rowcolor[gray]{.95}F40        & 0.61 (0.05) &\textbf{0.67 (0.01)} &0.64 (0.04) & \textbf{0.99 (0.01)} &0.52 (0.09) &0.67 (0.05)\\

\rowcolor[gray]{.95}F41                          & \textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} & \textbf{0.99 (0.01)} &0.26 (0.05) &0.50 (0.07)\\
\rowcolor[gray]{.95}F42        & 0.98 (0.01) &\textbf{1.00 (0.00)} &0.99 (0.00) & \textbf{0.98 (0.02)} &0.16 (0.03) &0.37 (0.05)\\
\rowcolor[gray]{.95}F43        & 0.99 (0.00) &\textbf{1.00 (0.00)} &\textbf{1.00 (0.01)} & \textbf{0.95 (0.06)} &0.15 (0.02) &0.35 (0.03)\\
\rowcolor[gray]{.95}F44                          & \textbf{1.00 (0.00)} &\textbf{1.00 (0.00) }&\textbf{1.00 (0.00)} & \textbf{0.99 (0.01)} &0.28 (0.05) &0.51 (0.10)\\
\rowcolor[gray]{.95}F45        & 0.93 (0.06) &\textbf{0.98 (0.02)} &0.95 (0.05) & \textbf{0.99 (0.01)} &0.36 (0.07) &0.58 (0.08)\\
\rowcolor[gray]{.95}F46        & 0.97 (0.01) &\textbf{1.00 (0.00)} &0.98 (0.01) & \textbf{0.99 (0.01)} &0.16 (0.03) &0.58 (0.15)\\
\rowcolor[gray]{.95}F47                 & 0.98 (0.00) &\textbf{1.00 (0.00)} &0.98 (0.00) & \textbf{0.99 (0.01)} &0.15 (0.03) &0.59 (0.15)\\
\rowcolor[gray]{.95}F48        & 0.98 (0.00) &\textbf{1.00 (0.00)} &0.98 (0.01) & \textbf{0.93 (0.13)} &0.15 (0.02) &0.39 (0.12)\\
\rowcolor[gray]{.95}F49        & 0.91 (0.05) &\textbf{0.97 (0.00)} &0.95 (0.03) & \textbf{0.98 (0.02)} &0.21 (0.03) &0.43 (0.10)\\
\rowcolor[gray]{.95}F50                 & 0.99 (0.00) &\textbf{1.00 (0.00)} &0.99 (0.00) & \textbf{0.99 (0.01)} &0.13 (0.02) &0.62 (0.10)\\
\rowcolor[gray]{.95}F51                 & \textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} &\textbf{1.00 (0.01)} & \textbf{0.97 (0.03)} &0.14 (0.02) &0.36 (0.08)\\
\rowcolor[gray]{.95}F52        & 0.90 (0.05) &\textbf{0.98 (0.01)} &0.97 (0.03) & \textbf{0.98 (0.02)} &0.16 (0.03) &0.44 (0.09)\\
\rowcolor[gray]{.95}F53                          & \textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} & \textbf{1.00 (0.01)} &0.37 (0.08) &0.61 (0.07)\\
\rowcolor[gray]{.95}F54        & 0.94 (0.06) &\textbf{0.97 (0.02)} &0.95 (0.03) & \textbf{1.00 (0.01)} &0.35 (0.05) &0.60 (0.06)\\
\rowcolor[gray]{.95}F55        & 0.22 (0.03) &\textbf{0.32 (0.04)} &0.22 (0.07) & \textbf{0.99 (0.01)} &0.87 (0.05) &0.95 (0.03)\\

\hline
Best/total &  31/73 & 57/73 & 43/73  &  73/73 & 2/73 & 1/73 \\
% \hline
\end{tabular}
\end{table}


==> files/nndom.tex <==
\begin{table}[tbp]
\centering
\small
\caption[Means and standard errors for proportion of nondominated solutions.]{Means and standard errors for proportion of nondominated solutions, for each problem. The best results are highlighted.}
\vspace{-1.1em}
\label{chap5:stats_bibbob_ndom}
\begin{tabular}[t]{c|c|c|c}
    \rowcolor[gray]{.8} \textbf{NNDOM} & MOEA/D-PS & Big population & Small population \\ \hline 
    
         
DTLZ1              & \textbf{1.00 (0.00) }&0.13 (0.08) &0.66 (0.25)\\
DTLZ2     & \textbf{0.99 (0.02)} &0.95 (0.02) &0.92 (0.05)\\
DTLZ3     & \textbf{0.99 (0.01)} &0.11 (0.13) &0.80 (0.20)\\
DTLZ4     & \textbf{0.99 (0.02)} &0.88 (0.05) &0.91 (0.05)\\

\rowcolor[gray]{.95}DTLZ1$^{-1}$ & \textbf{1.00 (0.00)} &0.29 (0.04) &0.98 (0.02)\\
\rowcolor[gray]{.95}DTLZ2$^{-1}$ & \textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} &\textbf{1.00 (0.01)}\\
\rowcolor[gray]{.95}DTLZ3$^{-1}$ & \textbf{1.00 (0.00)} &0.17 (0.03) &0.96 (0.03)\\
\rowcolor[gray]{.95}DTLZ4$^{-1}$ & \textbf{1.00 (0.00)} &\textbf{1.00 (0.00)} &0.99 (0.01)\\

UF1       & \textbf{0.96 (0.04)} &0.37 (0.06) &0.54 (0.07)\\
UF2       & \textbf{0.98 (0.03)} &0.38 (0.05) &0.54 (0.04)\\
UF3       & \textbf{0.97 (0.04)} &0.24 (0.03) &0.53 (0.09)\\
UF4       & \textbf{0.96 (0.04)} &0.56 (0.05) &0.73 (0.07)\\
UF5       & \textbf{0.78 (0.20)} &0.20 (0.03) &0.44 (0.10)\\
UF6       & \textbf{0.96 (0.04)} &0.31 (0.05) &0.50 (0.06)\\
UF7       & \textbf{0.93 (0.21)} &0.48 (0.08) &0.61 (0.11)\\
UF8       & \textbf{0.99 (0.01)} &0.64 (0.09) &0.79 (0.05)\\
UF9       & \textbf{0.99 (0.01)} &0.60 (0.12) &0.70 (0.10)\\
UF10      & \textbf{0.93 (0.08)} &0.46 (0.04) &0.73 (0.08)\\

\rowcolor[gray]{.95}F1         & \textbf{0.99 (0.01)} &0.32 (0.06) &0.50 (0.04)\\
\rowcolor[gray]{.95}F2         & \textbf{0.99 (0.01)} &0.29 (0.06) &0.54 (0.08)\\
\rowcolor[gray]{.95}F3         & \textbf{1.00 (0.01)} &0.36 (0.05) &0.58 (0.04)\\
\rowcolor[gray]{.95}F4         & \textbf{0.99 (0.01)} &0.25 (0.05) &0.47 (0.07)\\
\rowcolor[gray]{.95}F5         & \textbf{0.99 (0.01)} &0.33 (0.03) &0.49 (0.06)\\
\rowcolor[gray]{.95}F6         & \textbf{0.99 (0.01)} &0.25 (0.05) &0.51 (0.06)\\
\rowcolor[gray]{.95}F7         & \textbf{0.99 (0.01)} &0.18 (0.02) &0.37 (0.07)\\
\rowcolor[gray]{.95}F8         & \textbf{0.89 (0.11)} &0.16 (0.01) &0.42 (0.11)\\
\rowcolor[gray]{.95}F9         & \textbf{0.99 (0.01)} &0.31 (0.06) &0.54 (0.09)\\
\rowcolor[gray]{.95}F10        & \textbf{0.99 (0.01)} &0.45 (0.07) &0.55 (0.05)\\
\rowcolor[gray]{.95}F11        & \textbf{0.99 (0.01)} &0.31 (0.06) &0.55 (0.06)\\
\rowcolor[gray]{.95}F12        & \textbf{0.96 (0.04)} &0.29 (0.05) &0.62 (0.06)\\
\rowcolor[gray]{.95}F13        & \textbf{0.99 (0.01)} &0.27 (0.05) &0.53 (0.07)\\
\rowcolor[gray]{.95}F14        & \textbf{0.99 (0.02)} &0.30 (0.05) &0.48 (0.05)\\
\rowcolor[gray]{.95}F15        & \textbf{0.99 (0.01)} &0.28 (0.04) &0.49 (0.05)\\
\rowcolor[gray]{.95}F16        & \textbf{0.99 (0.01)} &0.17 (0.01) &0.41 (0.14)\\
\rowcolor[gray]{.95}F17        & \textbf{0.94 (0.05)} &0.15 (0.02) &0.39 (0.10)\\
\rowcolor[gray]{.95}F18        & \textbf{0.99 (0.01)} &0.31 (0.04) &0.54 (0.09)\\
\rowcolor[gray]{.95}F19        & \textbf{0.99 (0.02)} &0.40 (0.07) &0.62 (0.08)\\
\rowcolor[gray]{.95}F20        & \textbf{0.98 (0.02)} &0.43 (0.12) &0.66 (0.07)\\
\rowcolor[gray]{.95}F21        & \textbf{0.99 (0.02)} &0.28 (0.06) &0.56 (0.07)\\
\rowcolor[gray]{.95}F22        & \textbf{0.99 (0.02)} &0.33 (0.06) &0.55 (0.06)\\
\rowcolor[gray]{.95}F23        & \textbf{0.99 (0.01)} &0.31 (0.04) &0.54 (0.04)\\
\rowcolor[gray]{.95}F24        & \textbf{0.96 (0.04)} &0.16 (0.02) &0.39 (0.07)\\
\rowcolor[gray]{.95}F25        & \textbf{0.92 (0.10)} &0.14 (0.02) &0.32 (0.07)\\
\rowcolor[gray]{.95}F26        & \textbf{0.98 (0.02)} &0.37 (0.10) &0.70 (0.13)\\
\rowcolor[gray]{.95}F27        & \textbf{0.99 (0.01)} &0.37 (0.05) &0.62 (0.06)\\
\rowcolor[gray]{.95}F28        & \textbf{0.99 (0.02)} &0.24 (0.06) &0.47 (0.08)\\
\rowcolor[gray]{.95}F29        & \textbf{0.99 (0.02)} &0.24 (0.05) &0.44 (0.05)\\
\rowcolor[gray]{.95}F30        & \textbf{0.99 (0.02)} &0.27 (0.05) &0.45 (0.06)\\
\rowcolor[gray]{.95}F31        & \textbf{0.96 (0.07)} &0.16 (0.03) &0.42 (0.12)\\
\rowcolor[gray]{.95}F32        & \textbf{0.95 (0.06)} &0.14 (0.02) &0.34 (0.06)\\
\rowcolor[gray]{.95}F33        & \textbf{0.99 (0.02)} &0.25 (0.03) &0.56 (0.12)\\
\rowcolor[gray]{.95}F34        & \textbf{0.99 (0.02)} &0.35 (0.11) &0.50 (0.05)\\
\rowcolor[gray]{.95}F35        & \textbf{0.99 (0.01)} &0.40 (0.06) &0.55 (0.04)\\
\rowcolor[gray]{.95}F36        & \textbf{0.99 (0.01)} &0.30 (0.04) &0.52 (0.05)\\
\rowcolor[gray]{.95}F37        & \textbf{0.98 (0.02)} &0.21 (0.03) &0.42 (0.03)\\
\rowcolor[gray]{.95}F38        & \textbf{0.91 (0.12)} &0.18 (0.05) &0.39 (0.06)\\
\rowcolor[gray]{.95}F39        & \textbf{0.99 (0.01)} &0.33 (0.05) &0.53 (0.07)\\
\rowcolor[gray]{.95}F40        & \textbf{0.99 (0.01)} &0.52 (0.09) &0.67 (0.05)\\
\rowcolor[gray]{.95}F41        & \textbf{0.99 (0.01)} &0.26 (0.05) &0.50 (0.07)\\
\rowcolor[gray]{.95}F42        & \textbf{0.98 (0.02)} &0.16 (0.03) &0.37 (0.05)\\
\rowcolor[gray]{.95}F43        & \textbf{0.95 (0.06)} &0.15 (0.02) &0.35 (0.03)\\
\rowcolor[gray]{.95}F44        & \textbf{0.99 (0.01)} &0.28 (0.05) &0.51 (0.10)\\
\rowcolor[gray]{.95}F45        & \textbf{0.99 (0.01)} &0.36 (0.07) &0.58 (0.08)\\
\rowcolor[gray]{.95}F46        & \textbf{0.99 (0.01)} &0.16 (0.03) &0.58 (0.15)\\
\rowcolor[gray]{.95}F47        & \textbf{0.99 (0.01)} &0.15 (0.03) &0.59 (0.15)\\
\rowcolor[gray]{.95}F48        & \textbf{0.93 (0.13)} &0.15 (0.02) &0.39 (0.12)\\
\rowcolor[gray]{.95}F49        & \textbf{0.98 (0.02)} &0.21 (0.03) &0.43 (0.10)\\
\rowcolor[gray]{.95}F50        & \textbf{0.99 (0.01)} &0.13 (0.02) &0.62 (0.10)\\
\rowcolor[gray]{.95}F51        & \textbf{0.97 (0.03)} &0.14 (0.02) &0.36 (0.08)\\
\rowcolor[gray]{.95}F52        & \textbf{0.98 (0.02)} &0.16 (0.03) &0.44 (0.09)\\
\rowcolor[gray]{.95}F53        & \textbf{1.00 (0.01)} &0.37 (0.08) &0.61 (0.07)\\
\rowcolor[gray]{.95}F54        & \textbf{1.00 (0.01)} &0.35 (0.05) &0.60 (0.06)\\
\rowcolor[gray]{.95}F55        & \textbf{0.99 (0.01)} &0.87 (0.05) &0.95 (0.03)\\


\hline
Best/total &  73/73 & 2/73 & 1/73 \\

\end{tabular}
\end{table}

==> files/stats1.tex <==
\begin{table}[htbp]
	\centering
	\small
	\caption{Anytime Statistical significance of differences in median HV, for the three algorithms tested in this section, at 10000 function evaluations. Values are Hommel-adjusted p-values of Wilcoxon Rank-sum tests. ``$\uparrow$" indicates superiority of the column method and ``$\leftarrow$'' indicates superiority of the row method ($95\%$ confidence level).}
	\label{chap5:pvals1}

\begin{tabular}{l|ll}
		\hline
		\multicolumn{3}{c}{}\\\hline
		\rowcolor[gray]{.8}\multicolumn{3}{c}{\textbf{10000 function evaluations}}\\\hline
		\rowcolor[gray]{.95}\textbf{} & MOEA/D-PS & Big pop. \\ \hline
		Big pop.  & 2.452402e-03 $\uparrow$   &                    \\ \hline
		Small pop.  & 1.169062e-11 $\leftarrow$   & 2.488633e-10 $\leftarrow$   \\ 
		\hline
\end{tabular}
\end{table}


